Bidirectional Across Items, Sequential Within IDs: Hierarchy-Preserving Masked Discrete Diffusion for Generative Recommendation

Generative recommendation represents items with hierarchical semantic IDs (SIDs) and casts next-item prediction as sequence generation. Autoregressive language models preserve the coarse-to-fine order imposed by residual quantization but apply the same causal factorization across the interaction sequence. Masked discrete diffusion enables bidirectional learning across items; however, independently masking SID components can expose a fine residual code while hiding its required coarse prefix. We introduce Hierarchy-Preserving Diffusion (HPD), a masked discrete diffusion language modeling formulation that separates two dependency levels: (1) Across SIDs, full self-attention captures relations across the interaction sequence. (2) Within each SID, prefix-independent masking restricts each corrupted sequence to an observed prefix followed by a masked suffix. HPD combines this corruption with a training pipeline that first optimizes new SID-token embeddings and output weights with a fixed backbone and then jointly optimizes all parameters. Catalog-constrained beam search decodes the target SID from coarse to fine. HPD requires no task-specific architectural changes. Across three domains, Industrial and Scientific, Office Products, and Baby Products, we compare Qwen3-8B/LLaDA-8B-Base and Qwen2.5-7B/Dream-7B-Base autoregressive/diffusion large language model (AR-LLM/dLLM) pairs. At the final checkpoint, HPD achieves higher Hit Rate and NDCG than its matched AR-LLM at every evaluated cutoff. In the 8B LLaDA comparison, HPD obtains the best or tied-best score across all 18 metric--domain combinations. Comparisons with standard MDLM and DiffGRM evaluate HPD against alternative masked discrete diffusion objectives. An ablation shows that the proposed HPD pipeline outperforms the SID-token-only variant on every metric for Dream-7B-Base on Industrial and Scientific and LLaDA-8B-Base on Baby Products.

==> draft.tex <==
% Compact result cells for entries that include a secondary reported value.
\newcommand{\twolinescore}[2]{\shortstack{#1\\{\scriptsize (#2)}}}
\newcommand{\besttwolinescore}[2]{%
  \shortstack{\textbf{#1}\\{\scriptsize\textbf{(#2)}}}%
}

\begin{table}[t]
\centering
\caption{Recommendation results for the Qwen/LLaDA model pair on the Industrial and Office domains. Parenthesized numbers are the corresponding secondary values reported in the Industrial-domain experiments. The better result within each training-stage comparison is shown in \textbf{bold}.}
\label{tab:qwen_llada_results}
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llcccccc@{}}
\toprule
\textbf{Stage} & \textbf{Method}
& \textbf{HR@3} & \textbf{HR@5} & \textbf{HR@10}
& \textbf{NDCG@3} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Industrial domain}} \\
\addlinespace[2pt]
\multirow{2}{*}{Before}
& OpenOneRec (Qwen-8B)
& 0.0 & 0.00036 & 0.00124 & 0.0 & 0.00015 & 0.00043 \\
& Ours (LLaDA-8B-Base)
& 0.00053 & 0.00089 & 0.00213 & 0.00047 & 0.00062 & 0.00103 \\
\addlinespace[2pt]
\multirow{2}{*}{Stage 1}
& OpenOneRec (Qwen-8B)
& \twolinescore{0.0069}{0.00691}
& \twolinescore{0.0117}{0.01135}
& \twolinescore{0.0232}{0.02198}
& \twolinescore{0.0053}{0.00527}
& \twolinescore{0.0072}{0.00703}
& \twolinescore{0.0109}{0.010444} \\
& Ours (LLaDA-8B-Base)
& \besttwolinescore{0.0255}{0.02500}
& \besttwolinescore{0.0293}{0.02836}
& \besttwolinescore{0.0351}{0.03297}
& \besttwolinescore{0.0216}{0.02113}
& \besttwolinescore{0.0231}{0.02252}
& \besttwolinescore{0.0250}{0.02399} \\
\addlinespace[2pt]
\multirow{2}{*}{Stage 2}
& OpenOneRec (Qwen-8B)
& \twolinescore{0.00922}{0.00922}
& \twolinescore{0.01294}{0.01259}
& \twolinescore{0.02606}{0.02482}
& \twolinescore{0.00707}{0.00707}
& \twolinescore{0.00859}{0.00843}
& \twolinescore{0.012784}{0.01236} \\
& Ours (LLaDA-8B-Base)
& \besttwolinescore{0.02659}{0.02606}
& \besttwolinescore{0.03085}{0.02996}
& \besttwolinescore{0.03740}{0.03528}
& \besttwolinescore{0.02389}{0.02342}
& \besttwolinescore{0.02560}{0.02498}
& \besttwolinescore{0.02773}{0.02671} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Office domain}} \\
\addlinespace[2pt]
\multirow{2}{*}{Before}
& OpenOneRec (Qwen3-8B)
& & & & & & \\
& Ours (LLaDA-8B-Base)
& & & & & & \\
\addlinespace[2pt]
\multirow{2}{*}{Stage 1}
& OpenOneRec (Qwen3-8B)
& \textbf{0.00187} & \textbf{0.00296} & \textbf{0.00555}
& \textbf{0.00142} & \textbf{0.00187} & \textbf{0.00269} \\
& Ours (LLaDA-8B-Base)
& 0.00105 & 0.00173 & 0.00394 & 0.00068 & 0.00096 & 0.00166 \\
\addlinespace[2pt]
\multirow{2}{*}{Stage 2}
& OpenOneRec (Qwen3-8B)
& 0.00225 & 0.00364 & 0.00652 & 0.00163 & 0.00219 & 0.00311 \\
& Ours (LLaDA-8B-Base)
& \textbf{0.00595} & \textbf{0.00851} & \textbf{0.01340}
& \textbf{0.00465} & \textbf{0.00569} & \textbf{0.00727} \\
\bottomrule
\end{tabular}%
}
\end{table}

\begin{table}[t]
\centering
\caption{Recommendation results for the Qwen2.5-7B/Dream-7B-Base model pair on the Industrial and Office domains. Parenthesized numbers are the corresponding secondary values reported in the Industrial-domain experiments. The better result within each training-stage comparison is shown in \textbf{bold}.}
\label{tab:qwen_dream_results}
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llcccccc@{}}
\toprule
\textbf{Stage} & \textbf{Method}
& \textbf{HR@3} & \textbf{HR@5} & \textbf{HR@10}
& \textbf{NDCG@3} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Industrial domain}} \\
\addlinespace[2pt]
\multirow{2}{*}{Before}
& OpenOneRec (Qwen2.5-7B)
& 0.00053 & 0.00089 & 0.00248 & 0.00044 & 0.00060 & 0.00111 \\
& Ours (Dream-7B-Base)
& 0.0 & 0.00035 & 0.00124 & 0.0 & 0.00014 & 0.00040 \\
\addlinespace[2pt]
\multirow{2}{*}{Stage 1}
& OpenOneRec (Qwen2.5-7B)
& \twolinescore{0.01241}{0.01188}
& \twolinescore{0.01826}{0.01737}
& \twolinescore{0.02695}{0.02446}
& \twolinescore{0.00997}{0.00952}
& \twolinescore{0.01237}{0.01179}
& \twolinescore{0.01518}{0.01407} \\
& Ours (Dream-7B-Base)
& \besttwolinescore{0.04662}{0.04662}
& \besttwolinescore{0.05602}{0.05566}
& \besttwolinescore{0.07623}{0.07498}
& \besttwolinescore{0.04007}{0.04007}
& \besttwolinescore{0.04396}{0.04381}
& \besttwolinescore{0.05047}{0.05006} \\
\addlinespace[2pt]
\multirow{2}{*}{Stage 2}
& OpenOneRec (Qwen2.5-7B)
& \twolinescore{0.01844}{0.01844}
& \twolinescore{0.02358}{0.02322}
& \twolinescore{0.02854}{0.02730}
& \twolinescore{0.01519}{0.01519}
& \twolinescore{0.01732}{0.01717}
& \twolinescore{0.01891}{0.01848} \\
& Ours (Dream-7B-Base)
& \besttwolinescore{0.05052}{0.05052}
& \besttwolinescore{0.06435}{0.06399}
& \besttwolinescore{0.09059}{0.08935}
& \besttwolinescore{0.04166}{0.04166}
& \besttwolinescore{0.04738}{0.04724}
& \besttwolinescore{0.055849}{0.05545} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Office domain}} \\
\addlinespace[2pt]
\multirow{2}{*}{Before}
& OpenOneRec (Qwen2.5-7B)
& & & & & & \\
& Ours (Dream-7B-Base)
& & & & & & \\
\addlinespace[2pt]
\multirow{2}{*}{Stage 1}
& OpenOneRec (Qwen2.5-7B)
& 0.00135 & 0.00201 & 0.00326 & 0.00102 & 0.00129 & 0.00169 \\
& Ours (Dream-7B-Base)
& \textbf{0.00945} & \textbf{0.01303} & \textbf{0.01963}
& \textbf{0.00738} & \textbf{0.00885} & \textbf{0.01097} \\
\addlinespace[2pt]
\multirow{2}{*}{Stage 2}
& OpenOneRec (Qwen2.5-7B)
& 0.00179 & 0.00266 & 0.00459 & 0.00139 & 0.00175 & 0.00236 \\
& Ours (Dream-7B-Base)
& \textbf{0.03341} & \textbf{0.04085} & \textbf{0.05457}
& \textbf{0.02796} & \textbf{0.03102} & \textbf{0.03542} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/ablation_llada_industrial.tex <==
\begin{table}[t]
\centering
\caption{Training-scope ablation for HPD with LLaDA-8B-Base on Industrial
and Scientific. Performance immediately before the backbone is unfrozen is
compared with performance at the final checkpoint after training concludes
with all model parameters trainable. The better result in each column is shown
in \textbf{bold}.}
\label{tab:ablation_llada_industrial}
\small
\setlength{\tabcolsep}{3.5pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Trainable parameters}
& \textbf{HR@3} & \textbf{HR@5} & \textbf{HR@10}
& \textbf{NDCG@3} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
\midrule
SID embeddings/output weights
& 0.0255 & 0.0293 & 0.0351 & 0.0216 & 0.0231 & 0.0250 \\
All model parameters
& \textbf{0.0266} & \textbf{0.0309} & \textbf{0.0374}
& \textbf{0.0239} & \textbf{0.0256} & \textbf{0.0277} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/main_results_baby.tex <==
\begin{table}[t]
\centering
\caption{Final recommendation results on Baby Products for the 8B and 7B model pairs.}
\label{tab:main_results_baby}
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
\textbf{Method}
& \textbf{HR@3} & \textbf{HR@5} & \textbf{HR@10}
& \textbf{NDCG@3} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
\midrule
\multicolumn{7}{@{}l}{\textbf{8B Backbones}} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Base model}} \\
\addlinespace[1pt]
\hspace*{0.75em}Qwen3-8B
& 0.0003 & 0.0004 & 0.0007 & 0.0002 & 0.0003 & 0.0003 \\
\hspace*{0.75em}LLaDA-8B-Base
& 0.0006 & 0.0009 & 0.0013 & 0.0004 & 0.0006 & 0.0007 \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Trained}} \\
\addlinespace[1pt]
\multirow{2}{*}{\hspace*{0.75em}AR-LLM (Qwen3-8B)}
& 0.0021
& 0.0038
& 0.0069
& \underline{0.0014}
& 0.0022
& 0.0032 \\
& {\scriptsize (0.0018)}
& {\scriptsize (0.0034)}
& {\scriptsize (0.0062)}
& {\scriptsize\underline{(0.0012)}}
& {\scriptsize (0.0019)}
& {\scriptsize (0.0029)} \\
\multirow{2}{*}{\hspace*{0.75em}MDLM (LLaDA-8B-Base)}
& \underline{0.0092}
& \underline{0.0125}
& \underline{0.0202}
& \textbf{0.0074}
& \underline{0.0087}
& \underline{0.0112} \\
& {\scriptsize\underline{(0.0086)}}
& {\scriptsize\underline{(0.0116)}}
& {\scriptsize\underline{(0.0189)}}
& {\scriptsize\textbf{(0.0070)}}
& {\scriptsize\underline{(0.0081)}}
& {\scriptsize\underline{(0.0105)}} \\
\rowcolor[HTML]{F0F8FF}
& \textbf{0.0095}
& \textbf{0.0133}
& \textbf{0.0207}
& \textbf{0.0074}
& \textbf{0.0090}
& \textbf{0.0114} \\
\rowcolor[HTML]{F0F8FF}
\multirow{-2}{*}{\hspace*{0.75em}HPD (LLaDA-8B-Base)}
& {\scriptsize\textbf{(0.0089)}}
& {\scriptsize\textbf{(0.0124)}}
& {\scriptsize\textbf{(0.0194)}}
& {\scriptsize\textbf{(0.0070)}}
& {\scriptsize\textbf{(0.0084)}}
& {\scriptsize\textbf{(0.0107)}} \\
\midrule
\multicolumn{7}{@{}l}{\textbf{7B Backbones}} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Base model}} \\
\addlinespace[1pt]
\hspace*{0.75em}Qwen2.5-7B
& 0.0003 & 0.0004 & 0.0007 & 0.0002 & 0.0002 & 0.0003 \\
\hspace*{0.75em}Dream-7B-Base
& 0.0002 & 0.0003 & 0.0007 & 0.0002 & 0.0002 & 0.0003 \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Trained}} \\
\addlinespace[1pt]
\multirow{2}{*}{\hspace*{0.75em}AR-LLM (Qwen2.5-7B)}
& 0.0028 & 0.0039 & 0.0060 & 0.0022 & 0.0027 & 0.0033 \\
& {\scriptsize (0.0025)}
& {\scriptsize (0.0035)}
& {\scriptsize (0.0053)}
& {\scriptsize (0.0020)}
& {\scriptsize (0.0025)}
& {\scriptsize (0.0030)} \\
\multirow{2}{*}{\hspace*{0.75em}MDLM (Dream-7B-Base)}
& \textbf{0.0207}
& \textbf{0.0264}
& \textbf{0.0374}
& \textbf{0.0171}
& \textbf{0.0194}
& \textbf{0.0230} \\
& {\scriptsize\textbf{(0.0205)}}
& {\scriptsize\textbf{(0.0261)}}
& {\scriptsize\textbf{(0.0367)}}
& {\scriptsize\textbf{(0.0169)}}
& {\scriptsize\textbf{(0.0192)}}
& {\scriptsize\textbf{(0.0227)}} \\
\multirow{2}{*}{\hspace*{0.75em}DiffGRM (Dream-7B-Base)}
& 0.0050 & 0.0077 & 0.0125 & 0.0037 & 0.0048 & 0.0063 \\
& {\scriptsize (0.0048)}
& {\scriptsize (0.0074)}
& {\scriptsize (0.0118)}
& {\scriptsize (0.0035)}
& {\scriptsize (0.0046)}
& {\scriptsize (0.0060)} \\
\rowcolor[HTML]{F0F8FF}
& \underline{0.0178}
& \underline{0.0234}
& \underline{0.0331}
& \underline{0.0143}
& \underline{0.0167}
& \underline{0.0198} \\
\rowcolor[HTML]{F0F8FF}
\multirow{-2}{*}{\hspace*{0.75em}HPD (Dream-7B-Base)}
& {\scriptsize\underline{(0.0176)}}
& {\scriptsize\underline{(0.0231)}}
& {\scriptsize\underline{(0.0324)}}
& {\scriptsize\underline{(0.0141)}}
& {\scriptsize\underline{(0.0165)}}
& {\scriptsize\underline{(0.0195)}} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/main_results_industrial.tex <==
\begin{table}[t]
\centering
\caption{Final recommendation results on Industrial and Scientific for the 8B and 7B model pairs.}
\label{tab:main_results_industrial}
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
\textbf{Method}
& \textbf{HR@3} & \textbf{HR@5} & \textbf{HR@10}
& \textbf{NDCG@3} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
\midrule
\multicolumn{7}{@{}l}{\textbf{8B Backbones}} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Base model}} \\
\addlinespace[1pt]
\hspace*{0.75em}Qwen3-8B
& 0.0000 & 0.0004 & 0.0012 & 0.0000 & 0.0002 & 0.0004 \\
\hspace*{0.75em}LLaDA-8B-Base
& 0.0005 & 0.0009 & 0.0021 & 0.0005 & 0.0006 & 0.0010 \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Trained}} \\
\addlinespace[1pt]
\multirow{2}{*}{\hspace*{0.75em}AR-LLM (Qwen3-8B)}
& 0.0092 & 0.0129 & 0.0261 & 0.0071 & 0.0086 & 0.0128 \\
& {\scriptsize (0.0092)}
& {\scriptsize (0.0125)}
& {\scriptsize (0.0249)}
& {\scriptsize (0.0071)}
& {\scriptsize (0.0084)}
& {\scriptsize (0.0124)} \\
\multirow{2}{*}{\hspace*{0.75em}MDLM (LLaDA-8B-Base)}
& \underline{0.0161}
& \underline{0.0207}
& \underline{0.0289}
& \underline{0.0123}
& \underline{0.0142}
& \underline{0.0168} \\
& {\scriptsize\underline{(0.0156)}}
& {\scriptsize\underline{(0.0198)}}
& {\scriptsize\underline{(0.0268)}}
& {\scriptsize\underline{(0.0118)}}
& {\scriptsize\underline{(0.0136)}}
& {\scriptsize\underline{(0.0158)}} \\
\rowcolor[HTML]{F0F8FF}
& \textbf{0.0266}
& \textbf{0.0309}
& \textbf{0.0374}
& \textbf{0.0239}
& \textbf{0.0256}
& \textbf{0.0277} \\
\rowcolor[HTML]{F0F8FF}
\multirow{-2}{*}{\hspace*{0.75em}HPD (LLaDA-8B-Base)}
& {\scriptsize\textbf{(0.0261)}}
& {\scriptsize\textbf{(0.0300)}}
& {\scriptsize\textbf{(0.0353)}}
& {\scriptsize\textbf{(0.0234)}}
& {\scriptsize\textbf{(0.0250)}}
& {\scriptsize\textbf{(0.0267)}} \\
\midrule
\multicolumn{7}{@{}l}{\textbf{7B Backbones}} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Base model}} \\
\addlinespace[1pt]
\hspace*{0.75em}Qwen2.5-7B
& 0.0005 & 0.0009 & 0.0025 & 0.0004 & 0.0006 & 0.0011 \\
\hspace*{0.75em}Dream-7B-Base
& 0.0000 & 0.0004 & 0.0012 & 0.0000 & 0.0001 & 0.0004 \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Trained}} \\
\addlinespace[1pt]
\multirow{2}{*}{\hspace*{0.75em}AR-LLM (Qwen2.5-7B)}
& 0.0184 & 0.0236 & 0.0285 & 0.0152 & 0.0173 & 0.0189 \\
& {\scriptsize (0.0179)}
& {\scriptsize (0.0227)}
& {\scriptsize (0.0260)}
& {\scriptsize (0.0148)}
& {\scriptsize (0.0167)}
& {\scriptsize (0.0178)} \\
\multirow{2}{*}{\hspace*{0.75em}MDLM (Dream-7B-Base)}
& \textbf{0.0516}
& \underline{0.0633}
& \underline{0.0846}
& \textbf{0.0421}
& \underline{0.0468}
& \underline{0.0536} \\
& {\scriptsize\textbf{(0.0516)}}
& {\scriptsize\underline{(0.0629)}}
& {\scriptsize\underline{(0.0834)}}
& {\scriptsize\textbf{(0.0421)}}
& {\scriptsize\underline{(0.0467)}}
& {\scriptsize\underline{(0.0532)}} \\
\multirow{2}{*}{\hspace*{0.75em}DiffGRM (Dream-7B-Base)}
& 0.0434 & 0.0507 & 0.0605 & 0.0371 & 0.0401 & 0.0433 \\
& {\scriptsize (0.0434)}
& {\scriptsize (0.0503)}
& {\scriptsize (0.0593)}
& {\scriptsize (0.0371)}
& {\scriptsize (0.0400)}
& {\scriptsize (0.0429)} \\
\rowcolor[HTML]{F0F8FF}
& \underline{0.0505}
& \textbf{0.0644}
& \textbf{0.0906}
& \underline{0.0417}
& \textbf{0.0474}
& \textbf{0.0558} \\
\rowcolor[HTML]{F0F8FF}
\multirow{-2}{*}{\hspace*{0.75em}HPD (Dream-7B-Base)}
& {\scriptsize\underline{(0.0505)}}
& {\scriptsize\textbf{(0.0640)}}
& {\scriptsize\textbf{(0.0894)}}
& {\scriptsize\underline{(0.0417)}}
& {\scriptsize\textbf{(0.0473)}}
& {\scriptsize\textbf{(0.0554)}} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/main_results_office.tex <==
\begin{table}[t]
\centering
\caption{Final recommendation results on Office Products for the 8B and 7B model pairs.}
\label{tab:main_results_office}
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
\textbf{Method}
& \textbf{HR@3} & \textbf{HR@5} & \textbf{HR@10}
& \textbf{NDCG@3} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
\midrule
\multicolumn{7}{@{}l}{\textbf{8B Backbones}} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Base model}} \\
\addlinespace[1pt]
\hspace*{0.75em}Qwen3-8B
& 0.0002 & 0.0004 & 0.0008 & 0.0002 & 0.0002 & 0.0004 \\
\hspace*{0.75em}LLaDA-8B-Base
& 0.0001 & 0.0002 & 0.0004 & 0.0001 & 0.0001 & 0.0002 \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Trained}} \\
\addlinespace[1pt]
\multirow{2}{*}{\hspace*{0.75em}AR-LLM (Qwen3-8B)}
& 0.0023 & 0.0036 & 0.0065 & 0.0016 & 0.0022 & 0.0031 \\
& {\scriptsize (0.0021)}
& {\scriptsize (0.0032)}
& {\scriptsize (0.0057)}
& {\scriptsize (0.0014)}
& {\scriptsize (0.0020)}
& {\scriptsize (0.0027)} \\
\multirow{2}{*}{\hspace*{0.75em}MDLM (LLaDA-8B-Base)}
& \underline{0.0053}
& \underline{0.0075}
& \underline{0.0124}
& \underline{0.0040}
& \underline{0.0049}
& \underline{0.0064} \\
& {\scriptsize\underline{(0.0052)}}
& {\scriptsize\underline{(0.0073)}}
& {\scriptsize\underline{(0.0120)}}
& {\scriptsize\underline{(0.0039)}}
& {\scriptsize\underline{(0.0048)}}
& {\scriptsize\underline{(0.0062)}} \\
\rowcolor[HTML]{F0F8FF}
& \textbf{0.0060}
& \textbf{0.0085}
& \textbf{0.0134}
& \textbf{0.0047}
& \textbf{0.0057}
& \textbf{0.0073} \\
\rowcolor[HTML]{F0F8FF}
\multirow{-2}{*}{\hspace*{0.75em}HPD (LLaDA-8B-Base)}
& {\scriptsize\textbf{(0.0059)}}
& {\scriptsize\textbf{(0.0083)}}
& {\scriptsize\textbf{(0.0130)}}
& {\scriptsize\textbf{(0.0046)}}
& {\scriptsize\textbf{(0.0056)}}
& {\scriptsize\textbf{(0.0071)}} \\
\midrule
\multicolumn{7}{@{}l}{\textbf{7B Backbones}} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Base model}} \\
\addlinespace[1pt]
\hspace*{0.75em}Qwen2.5-7B
& 0.0001 & 0.0002 & 0.0005 & 0.0001 & 0.0001 & 0.0002 \\
\hspace*{0.75em}Dream-7B-Base
& 0.0001 & 0.0002 & 0.0004 & 0.0001 & 0.0001 & 0.0002 \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Trained}} \\
\addlinespace[1pt]
\multirow{2}{*}{\hspace*{0.75em}AR-LLM (Qwen2.5-7B)}
& 0.0018 & 0.0027 & 0.0046 & 0.0014 & 0.0018 & 0.0024 \\
& {\scriptsize (0.0017)}
& {\scriptsize (0.0025)}
& {\scriptsize (0.0041)}
& {\scriptsize (0.0013)}
& {\scriptsize (0.0017)}
& {\scriptsize (0.0022)} \\
\multirow{2}{*}{\hspace*{0.75em}MDLM (Dream-7B-Base)}
& \textbf{0.0367}
& \textbf{0.0446}
& \textbf{0.0573}
& \textbf{0.0319}
& \textbf{0.0352}
& \textbf{0.0393} \\
& {\scriptsize\textbf{(0.0366)}}
& {\scriptsize\textbf{(0.0444)}}
& {\scriptsize\textbf{(0.0569)}}
& {\scriptsize\textbf{(0.0318)}}
& {\scriptsize\textbf{(0.0351)}}
& {\scriptsize\textbf{(0.0391)}} \\
\multirow{2}{*}{\hspace*{0.75em}DiffGRM (Dream-7B-Base)}
& 0.0098 & 0.0130 & 0.0194 & 0.0074 & 0.0088 & 0.0108 \\
& {\scriptsize (0.0097)}
& {\scriptsize (0.0128)}
& {\scriptsize (0.0190)}
& {\scriptsize (0.0073)}
& {\scriptsize (0.0087)}
& {\scriptsize (0.0106)} \\
\rowcolor[HTML]{F0F8FF}
& \underline{0.0334}
& \underline{0.0409}
& \underline{0.0546}
& \underline{0.0280}
& \underline{0.0310}
& \underline{0.0354} \\
\rowcolor[HTML]{F0F8FF}
\multirow{-2}{*}{\hspace*{0.75em}HPD (Dream-7B-Base)}
& {\scriptsize\underline{(0.0333)}}
& {\scriptsize\underline{(0.0407)}}
& {\scriptsize\underline{(0.0542)}}
& {\scriptsize\underline{(0.0279)}}
& {\scriptsize\underline{(0.0309)}}
& {\scriptsize\underline{(0.0352)}} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/qwen25_dream.tex <==
\begin{table}[t]
\centering
\caption{Recommendation results for the Qwen2.5/Dream model pair on the Industrial and Scientific, Office Products, and Baby Products domains. \emph{Before} denotes inference immediately after adding the new SID tokens to the model's embedding and output spaces, prior to recommendation training. For each trained model, the smaller parenthesized value is the difference from its corresponding \emph{Before} score; positive values denote improvement. The best and second-best distinct scores within each domain and training scope are shown in \textbf{bold} and with \underline{underlining}, respectively; ties receive the same emphasis. All trained results use the checkpoint saved at update 1,000.}
\label{tab:qwen_dream_results}
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}clcccccc@{}}
\toprule
\textbf{Training scope} & \textbf{Method}
& \textbf{HR@3} & \textbf{HR@5} & \textbf{HR@10}
& \textbf{NDCG@3} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Industrial and Scientific}} \\
\addlinespace[2pt]
\multirow{2}{*}{Before}
& AR-LLM (Qwen2.5-7B)
& 0.0005 & 0.0009 & 0.0025 & 0.0004 & 0.0006 & 0.0011 \\
& dLLM (Dream-7B-Base)
& 0.0000 & 0.0004 & 0.0012 & 0.0000 & 0.0001 & 0.0004 \\
\addlinespace[2pt]
\multirow{8}{*}{SID parameters only}
& \multirow{2}{*}{AR-LLM (Qwen2.5-7B)}
& 0.0124
& 0.0183
& 0.0270
& 0.0100
& 0.0124
& 0.0152 \\
&
& {\scriptsize (0.0119)}
& {\scriptsize (0.0174)}
& {\scriptsize (0.0245)}
& {\scriptsize (0.0096)}
& {\scriptsize (0.0118)}
& {\scriptsize (0.0141)} \\
& \multirow{2}{*}{HPD (Dream-7B-Base)}
& \underline{0.0466}
& \underline{0.0560}
& \textbf{0.0762}
& \underline{0.0401}
& \underline{0.0440}
& \underline{0.0505} \\
&
& {\scriptsize\underline{(0.0466)}}
& {\scriptsize\underline{(0.0556)}}
& {\scriptsize\textbf{(0.0750)}}
& {\scriptsize\underline{(0.0401)}}
& {\scriptsize\underline{(0.0439)}}
& {\scriptsize\underline{(0.0501)}} \\
& \multirow{2}{*}{MDLM (Dream-7B-Base)}
& \textbf{0.0491}
& \textbf{0.0597}
& \underline{0.0757}
& \textbf{0.0424}
& \textbf{0.0467}
& \textbf{0.0518} \\
&
& {\scriptsize\textbf{(0.0491)}}
& {\scriptsize\textbf{(0.0593)}}
& {\scriptsize\underline{(0.0745)}}
& {\scriptsize\textbf{(0.0424)}}
& {\scriptsize\textbf{(0.0466)}}
& {\scriptsize\textbf{(0.0514)}} \\
& \multirow{2}{*}{DiffGRM (Dream-7B-Base)}
& 0.0298
& 0.0452
& 0.0667
& 0.0215
& 0.0278
& 0.0347 \\
&
& {\scriptsize (0.0298)}
& {\scriptsize (0.0448)}
& {\scriptsize (0.0655)}
& {\scriptsize (0.0215)}
& {\scriptsize (0.0277)}
& {\scriptsize (0.0343)} \\
\addlinespace[2pt]
\multirow{8}{*}{All model parameters}
& \multirow{2}{*}{AR-LLM (Qwen2.5-7B)}
& 0.0184
& 0.0236
& 0.0285
& 0.0152
& 0.0173
& 0.0189 \\
&
& {\scriptsize (0.0179)}
& {\scriptsize (0.0227)}
& {\scriptsize (0.0260)}
& {\scriptsize (0.0148)}
& {\scriptsize (0.0167)}
& {\scriptsize (0.0178)} \\
& \multirow{2}{*}{HPD (Dream-7B-Base)}
& \underline{0.0505}
& \textbf{0.0644}
& \textbf{0.0906}
& \underline{0.0417}
& \textbf{0.0474}
& \textbf{0.0558} \\
&
& {\scriptsize\underline{(0.0505)}}
& {\scriptsize\textbf{(0.0640)}}
& {\scriptsize\textbf{(0.0894)}}
& {\scriptsize\underline{(0.0417)}}
& {\scriptsize\textbf{(0.0473)}}
& {\scriptsize\textbf{(0.0554)}} \\
& \multirow{2}{*}{MDLM (Dream-7B-Base)}
& \textbf{0.0516}
& \underline{0.0633}
& \underline{0.0846}
& \textbf{0.0421}
& \underline{0.0468}
& \underline{0.0536} \\
&
& {\scriptsize\textbf{(0.0516)}}
& {\scriptsize\underline{(0.0629)}}
& {\scriptsize\underline{(0.0834)}}
& {\scriptsize\textbf{(0.0421)}}
& {\scriptsize\underline{(0.0467)}}
& {\scriptsize\underline{(0.0532)}} \\
& \multirow{2}{*}{DiffGRM (Dream-7B-Base)}
& 0.0434
& 0.0507
& 0.0605
& 0.0371
& 0.0401
& 0.0433 \\
&
& {\scriptsize (0.0434)}
& {\scriptsize (0.0503)}
& {\scriptsize (0.0593)}
& {\scriptsize (0.0371)}
& {\scriptsize (0.0400)}
& {\scriptsize (0.0429)} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Office Products}} \\
\addlinespace[2pt]
\multirow{2}{*}{Before}
& AR-LLM (Qwen2.5-7B)
& 0.0001 & 0.0002 & 0.0005 & 0.0001 & 0.0001 & 0.0002 \\
& dLLM (Dream-7B-Base)
& 0.0001 & 0.0002 & 0.0004 & 0.0001 & 0.0001 & 0.0002 \\
\addlinespace[2pt]
\multirow{8}{*}{SID parameters only}
& \multirow{2}{*}{AR-LLM (Qwen2.5-7B)}
& 0.0014
& 0.0020
& 0.0033
& 0.0010
& 0.0013
& 0.0017 \\
&
& {\scriptsize (0.0013)}
& {\scriptsize (0.0018)}
& {\scriptsize (0.0028)}
& {\scriptsize (0.0009)}
& {\scriptsize (0.0012)}
& {\scriptsize (0.0015)} \\
& \multirow{2}{*}{HPD (Dream-7B-Base)}
& \textbf{0.0095}
& \textbf{0.0130}
& \textbf{0.0196}
& \textbf{0.0074}
& \textbf{0.0089}
& \textbf{0.0110} \\
&
& {\scriptsize\textbf{(0.0094)}}
& {\scriptsize\textbf{(0.0128)}}
& {\scriptsize\textbf{(0.0192)}}
& {\scriptsize\textbf{(0.0073)}}
& {\scriptsize\textbf{(0.0088)}}
& {\scriptsize\textbf{(0.0108)}} \\
& \multirow{2}{*}{MDLM (Dream-7B-Base)}
& \underline{0.0080}
& \underline{0.0104}
& \underline{0.0153}
& \underline{0.0064}
& \underline{0.0074}
& \underline{0.0090} \\
&
& {\scriptsize\underline{(0.0079)}}
& {\scriptsize\underline{(0.0102)}}
& {\scriptsize\underline{(0.0149)}}
& {\scriptsize\underline{(0.0063)}}
& {\scriptsize\underline{(0.0073)}}
& {\scriptsize\underline{(0.0088)}} \\
& \multirow{2}{*}{DiffGRM (Dream-7B-Base)}
& 0.0073
& 0.0098
& 0.0145
& 0.0057
& 0.0067
& 0.0082 \\
&
& {\scriptsize (0.0072)}
& {\scriptsize (0.0096)}
& {\scriptsize (0.0141)}
& {\scriptsize (0.0056)}
& {\scriptsize (0.0066)}
& {\scriptsize (0.0080)} \\
\addlinespace[2pt]
\multirow{8}{*}{All model parameters}
& \multirow{2}{*}{AR-LLM (Qwen2.5-7B)}
& 0.0018
& 0.0027
& 0.0046
& 0.0014
& 0.0018
& 0.0024 \\
&
& {\scriptsize (0.0017)}
& {\scriptsize (0.0025)}
& {\scriptsize (0.0041)}
& {\scriptsize (0.0013)}
& {\scriptsize (0.0017)}
& {\scriptsize (0.0022)} \\
& \multirow{2}{*}{HPD (Dream-7B-Base)}
& \underline{0.0334}
& \underline{0.0409}
& \underline{0.0546}
& \underline{0.0280}
& \underline{0.0310}
& \underline{0.0354} \\
&
& {\scriptsize\underline{(0.0333)}}
& {\scriptsize\underline{(0.0407)}}
& {\scriptsize\underline{(0.0542)}}
& {\scriptsize\underline{(0.0279)}}
& {\scriptsize\underline{(0.0309)}}
& {\scriptsize\underline{(0.0352)}} \\
& \multirow{2}{*}{MDLM (Dream-7B-Base)}
& \textbf{0.0367}
& \textbf{0.0446}
& \textbf{0.0573}
& \textbf{0.0319}
& \textbf{0.0352}
& \textbf{0.0393} \\
&
& {\scriptsize\textbf{(0.0366)}}
& {\scriptsize\textbf{(0.0444)}}
& {\scriptsize\textbf{(0.0569)}}
& {\scriptsize\textbf{(0.0318)}}
& {\scriptsize\textbf{(0.0351)}}
& {\scriptsize\textbf{(0.0391)}} \\
& \multirow{2}{*}{DiffGRM (Dream-7B-Base)}
& 0.0098
& 0.0130
& 0.0194
& 0.0074
& 0.0088
& 0.0108 \\
&
& {\scriptsize (0.0097)}
& {\scriptsize (0.0128)}
& {\scriptsize (0.0190)}
& {\scriptsize (0.0073)}
& {\scriptsize (0.0087)}
& {\scriptsize (0.0106)} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Baby Products}} \\
\addlinespace[2pt]
\multirow{2}{*}{Before}
& AR-LLM (Qwen2.5-7B)
& 0.0003 & 0.0004 & 0.0007 & 0.0002 & 0.0002 & 0.0003 \\
& dLLM (Dream-7B-Base)
& 0.0002 & 0.0003 & 0.0007 & 0.0002 & 0.0002 & 0.0003 \\
\addlinespace[2pt]
\multirow{8}{*}{SID parameters only}
& \multirow{2}{*}{AR-LLM (Qwen2.5-7B)}
& 0.0019
& 0.0029
& 0.0044
& 0.0015
& 0.0019
& 0.0024 \\
&
& {\scriptsize (0.0016)}
& {\scriptsize (0.0025)}
& {\scriptsize (0.0037)}
& {\scriptsize (0.0013)}
& {\scriptsize (0.0017)}
& {\scriptsize (0.0021)} \\
& \multirow{2}{*}{HPD (Dream-7B-Base)}
& \textbf{0.0102}
& \textbf{0.0148}
& \textbf{0.0237}
& \textbf{0.0077}
& \textbf{0.0096}
& \textbf{0.0125} \\
&
& {\scriptsize\textbf{(0.0100)}}
& {\scriptsize\textbf{(0.0145)}}
& {\scriptsize\textbf{(0.0230)}}
& {\scriptsize\textbf{(0.0075)}}
& {\scriptsize\textbf{(0.0094)}}
& {\scriptsize\textbf{(0.0122)}} \\
& \multirow{2}{*}{MDLM (Dream-7B-Base)}
& \underline{0.0073}
& \underline{0.0108}
& \underline{0.0177}
& \underline{0.0055}
& \underline{0.0069}
& \underline{0.0092} \\
&
& {\scriptsize\underline{(0.0071)}}
& {\scriptsize\underline{(0.0105)}}
& {\scriptsize\underline{(0.0170)}}
& {\scriptsize\underline{(0.0053)}}
& {\scriptsize\underline{(0.0067)}}
& {\scriptsize\underline{(0.0089)}} \\
& \multirow{2}{*}{DiffGRM (Dream-7B-Base)}
& 0.0065
& 0.0099
& 0.0166
& 0.0048
& 0.0062
& 0.0083 \\
&
& {\scriptsize (0.0063)}
& {\scriptsize (0.0096)}
& {\scriptsize (0.0159)}
& {\scriptsize (0.0046)}
& {\scriptsize (0.0060)}
& {\scriptsize (0.0080)} \\
\addlinespace[2pt]
\multirow{8}{*}{All model parameters}
& \multirow{2}{*}{AR-LLM (Qwen2.5-7B)}
& 0.0028
& 0.0039
& 0.0060
& 0.0022
& 0.0027
& 0.0033 \\
&
& {\scriptsize (0.0025)}
& {\scriptsize (0.0035)}
& {\scriptsize (0.0053)}
& {\scriptsize (0.0020)}
& {\scriptsize (0.0025)}
& {\scriptsize (0.0030)} \\
& \multirow{2}{*}{HPD (Dream-7B-Base)}
& \underline{0.0178}
& \underline{0.0234}
& \underline{0.0331}
& \underline{0.0143}
& \underline{0.0167}
& \underline{0.0198} \\
&
& {\scriptsize\underline{(0.0176)}}
& {\scriptsize\underline{(0.0231)}}
& {\scriptsize\underline{(0.0324)}}
& {\scriptsize\underline{(0.0141)}}
& {\scriptsize\underline{(0.0165)}}
& {\scriptsize\underline{(0.0195)}} \\
& \multirow{2}{*}{MDLM (Dream-7B-Base)}
& \textbf{0.0207}
& \textbf{0.0264}
& \textbf{0.0374}
& \textbf{0.0171}
& \textbf{0.0194}
& \textbf{0.0230} \\
&
& {\scriptsize\textbf{(0.0205)}}
& {\scriptsize\textbf{(0.0261)}}
& {\scriptsize\textbf{(0.0367)}}
& {\scriptsize\textbf{(0.0169)}}
& {\scriptsize\textbf{(0.0192)}}
& {\scriptsize\textbf{(0.0227)}} \\
& \multirow{2}{*}{DiffGRM (Dream-7B-Base)}
& 0.0050
& 0.0077
& 0.0125
& 0.0037
& 0.0048
& 0.0063 \\
&
& {\scriptsize (0.0048)}
& {\scriptsize (0.0074)}
& {\scriptsize (0.0118)}
& {\scriptsize (0.0035)}
& {\scriptsize (0.0046)}
& {\scriptsize (0.0060)} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/qwen25_dream_stage1.tex <==
\begin{table}[t]
\centering
\caption{Recommendation results for the Qwen2.5/Dream model pair before recommendation training and after training only the SID-token embeddings and output weights on the Industrial and Scientific, Office Products, and Baby Products domains. Parenthesized values for trained models are differences from the corresponding base-model results. The best trained score within each domain is shown in \textbf{bold}. All trained results use the checkpoint saved at update 1,000.}
\label{tab:qwen_dream_stage1_results}
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}clcccccc@{}}
\toprule
\textbf{Training scope} & \textbf{Method}
& \textbf{HR@3} & \textbf{HR@5} & \textbf{HR@10}
& \textbf{NDCG@3} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Industrial and Scientific}} \\
\addlinespace[2pt]
\multirow{2}{*}{Before}
& OpenOneRec (Qwen2.5-7B)
& 0.0005 & 0.0009 & 0.0025 & 0.0004 & 0.0006 & 0.0011 \\
& Ours (Dream-7B-Base)
& 0.0000 & 0.0004 & 0.0012 & 0.0000 & 0.0001 & 0.0004 \\
\addlinespace[2pt]
\multirow{8}{*}{SID parameters only}
& \multirow{2}{*}{OpenOneRec (Qwen2.5-7B)}
& 0.0124
& 0.0183
& 0.0270
& 0.0100
& 0.0124
& 0.0152 \\
&
& {\scriptsize (0.0119)}
& {\scriptsize (0.0174)}
& {\scriptsize (0.0245)}
& {\scriptsize (0.0096)}
& {\scriptsize (0.0118)}
& {\scriptsize (0.0141)} \\
& \multirow{2}{*}{Ours (Dream-7B-Base)}
& 0.0466
& 0.0560
& \textbf{0.0762}
& 0.0401
& 0.0440
& 0.0505 \\
&
& {\scriptsize (0.0466)}
& {\scriptsize (0.0556)}
& {\scriptsize\textbf{(0.0750)}}
& {\scriptsize (0.0401)}
& {\scriptsize (0.0439)}
& {\scriptsize (0.0501)} \\
& \multirow{2}{*}{Original Diffusion (Dream-7B-Base)}
& \textbf{0.0491}
& \textbf{0.0597}
& 0.0757
& \textbf{0.0424}
& \textbf{0.0467}
& \textbf{0.0518} \\
&
& {\scriptsize\textbf{(0.0491)}}
& {\scriptsize\textbf{(0.0593)}}
& {\scriptsize (0.0745)}
& {\scriptsize\textbf{(0.0424)}}
& {\scriptsize\textbf{(0.0466)}}
& {\scriptsize\textbf{(0.0514)}} \\
& \multirow{2}{*}{DiffGRM (Dream-7B-Base)}
& 0.0298
& 0.0452
& 0.0667
& 0.0215
& 0.0278
& 0.0347 \\
&
& {\scriptsize (0.0298)}
& {\scriptsize (0.0448)}
& {\scriptsize (0.0655)}
& {\scriptsize (0.0215)}
& {\scriptsize (0.0277)}
& {\scriptsize (0.0343)} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Office Products}} \\
\addlinespace[2pt]
\multirow{2}{*}{Before}
& OpenOneRec (Qwen2.5-7B)
& 0.0001 & 0.0002 & 0.0005 & 0.0001 & 0.0001 & 0.0002 \\
& Ours (Dream-7B-Base)
& 0.0001 & 0.0002 & 0.0004 & 0.0001 & 0.0001 & 0.0002 \\
\addlinespace[2pt]
\multirow{8}{*}{SID parameters only}
& \multirow{2}{*}{OpenOneRec (Qwen2.5-7B)}
& 0.0014
& 0.0020
& 0.0033
& 0.0010
& 0.0013
& 0.0017 \\
&
& {\scriptsize (0.0013)}
& {\scriptsize (0.0018)}
& {\scriptsize (0.0028)}
& {\scriptsize (0.0009)}
& {\scriptsize (0.0012)}
& {\scriptsize (0.0015)} \\
& \multirow{2}{*}{Ours (Dream-7B-Base)}
& \textbf{0.0095}
& \textbf{0.0130}
& \textbf{0.0196}
& \textbf{0.0074}
& \textbf{0.0089}
& \textbf{0.0110} \\
&
& {\scriptsize\textbf{(0.0094)}}
& {\scriptsize\textbf{(0.0128)}}
& {\scriptsize\textbf{(0.0192)}}
& {\scriptsize\textbf{(0.0073)}}
& {\scriptsize\textbf{(0.0088)}}
& {\scriptsize\textbf{(0.0108)}} \\
& \multirow{2}{*}{Original Diffusion (Dream-7B-Base)}
& 0.0080
& 0.0104
& 0.0153
& 0.0064
& 0.0074
& 0.0090 \\
&
& {\scriptsize (0.0079)}
& {\scriptsize (0.0102)}
& {\scriptsize (0.0149)}
& {\scriptsize (0.0063)}
& {\scriptsize (0.0073)}
& {\scriptsize (0.0088)} \\
& \multirow{2}{*}{DiffGRM (Dream-7B-Base)}
& 0.0073
& 0.0098
& 0.0145
& 0.0057
& 0.0067
& 0.0082 \\
&
& {\scriptsize (0.0072)}
& {\scriptsize (0.0096)}
& {\scriptsize (0.0141)}
& {\scriptsize (0.0056)}
& {\scriptsize (0.0066)}
& {\scriptsize (0.0080)} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Baby Products}} \\
\addlinespace[2pt]
\multirow{2}{*}{Before}
& OpenOneRec (Qwen2.5-7B)
& 0.0003 & 0.0004 & 0.0007 & 0.0002 & 0.0002 & 0.0003 \\
& Ours (Dream-7B-Base)
& 0.0002 & 0.0003 & 0.0007 & 0.0002 & 0.0002 & 0.0003 \\
\addlinespace[2pt]
\multirow{8}{*}{SID parameters only}
& \multirow{2}{*}{OpenOneRec (Qwen2.5-7B)}
& 0.0019
& 0.0029
& 0.0044
& 0.0015
& 0.0019
& 0.0024 \\
&
& {\scriptsize (0.0016)}
& {\scriptsize (0.0025)}
& {\scriptsize (0.0037)}
& {\scriptsize (0.0013)}
& {\scriptsize (0.0017)}
& {\scriptsize (0.0021)} \\
& \multirow{2}{*}{Ours (Dream-7B-Base)}
& \textbf{0.0102}
& \textbf{0.0148}
& \textbf{0.0237}
& \textbf{0.0077}
& \textbf{0.0096}
& \textbf{0.0125} \\
&
& {\scriptsize\textbf{(0.0100)}}
& {\scriptsize\textbf{(0.0145)}}
& {\scriptsize\textbf{(0.0230)}}
& {\scriptsize\textbf{(0.0075)}}
& {\scriptsize\textbf{(0.0094)}}
& {\scriptsize\textbf{(0.0122)}} \\
& \multirow{2}{*}{Original Diffusion (Dream-7B-Base)}
& 0.0073
& 0.0108
& 0.0177
& 0.0055
& 0.0069
& 0.0092 \\
&
& {\scriptsize (0.0071)}
& {\scriptsize (0.0105)}
& {\scriptsize (0.0170)}
& {\scriptsize (0.0053)}
& {\scriptsize (0.0067)}
& {\scriptsize (0.0089)} \\
& \multirow{2}{*}{DiffGRM (Dream-7B-Base)}
& 0.0065
& 0.0099
& 0.0166
& 0.0048
& 0.0062
& 0.0083 \\
&
& {\scriptsize (0.0063)}
& {\scriptsize (0.0096)}
& {\scriptsize (0.0159)}
& {\scriptsize (0.0046)}
& {\scriptsize (0.0060)}
& {\scriptsize (0.0080)} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/qwen25_dream_stage2.tex <==
\begin{table}[h]
\centering
\caption{Final recommendation results for the Qwen2.5/Dream model pair.}
\label{tab:qwen_dream_final_results}
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.15}
% Set the numeric factor to the desired width; 0.8 means 80% of \linewidth.
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
\textbf{Method}
& \textbf{HR@3} & \textbf{HR@5} & \textbf{HR@10}
& \textbf{NDCG@3} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
\midrule
\multicolumn{7}{@{}l}{\textbf{Industrial and Scientific}} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Base model}} \\
\addlinespace[1pt]
\hspace*{0.75em}Qwen2.5-7B
& 0.0005 & 0.0009 & 0.0025 & 0.0004 & 0.0006 & 0.0011 \\
\hspace*{0.75em}Dream-7B-Base
& 0.0000 & 0.0004 & 0.0012 & 0.0000 & 0.0001 & 0.0004 \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Trained}} \\
\addlinespace[1pt]
\multirow{2}{*}{\hspace*{0.75em}AR-LLM (Qwen2.5-7B)}
& 0.0184
& 0.0236
& 0.0285
& 0.0152
& 0.0173
& 0.0189 \\
& {\scriptsize (0.0179)}
& {\scriptsize (0.0227)}
& {\scriptsize (0.0260)}
& {\scriptsize (0.0148)}
& {\scriptsize (0.0167)}
& {\scriptsize (0.0178)} \\
\multirow{2}{*}{\hspace*{0.75em}MDLM (Dream-7B-Base)}
& \textbf{0.0516}
& \underline{0.0633}
& \underline{0.0846}
& \textbf{0.0421}
& \underline{0.0468}
& \underline{0.0536} \\
& {\scriptsize\textbf{(0.0516)}}
& {\scriptsize\underline{(0.0629)}}
& {\scriptsize\underline{(0.0834)}}
& {\scriptsize\textbf{(0.0421)}}
& {\scriptsize\underline{(0.0467)}}
& {\scriptsize\underline{(0.0532)}} \\
\multirow{2}{*}{\hspace*{0.75em}DiffGRM (Dream-7B-Base)}
& 0.0434
& 0.0507
& 0.0605
& 0.0371
& 0.0401
& 0.0433 \\
& {\scriptsize (0.0434)}
& {\scriptsize (0.0503)}
& {\scriptsize (0.0593)}
& {\scriptsize (0.0371)}
& {\scriptsize (0.0400)}
& {\scriptsize (0.0429)} \\
\rowcolor[HTML]{F0F8FF}
& \underline{0.0505}
& \textbf{0.0644}
& \textbf{0.0906}
& \underline{0.0417}
& \textbf{0.0474}
& \textbf{0.0558} \\
\rowcolor[HTML]{F0F8FF}
\multirow{-2}{*}{\hspace*{0.75em}HPD (Dream-7B-Base)}
& {\scriptsize\underline{(0.0505)}}
& {\scriptsize\textbf{(0.0640)}}
& {\scriptsize\textbf{(0.0894)}}
& {\scriptsize\underline{(0.0417)}}
& {\scriptsize\textbf{(0.0473)}}
& {\scriptsize\textbf{(0.0554)}} \\
\midrule
\multicolumn{7}{@{}l}{\textbf{Office Products}} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Base model}} \\
\addlinespace[1pt]
\hspace*{0.75em}Qwen2.5-7B
& 0.0001 & 0.0002 & 0.0005 & 0.0001 & 0.0001 & 0.0002 \\
\hspace*{0.75em}Dream-7B-Base
& 0.0001 & 0.0002 & 0.0004 & 0.0001 & 0.0001 & 0.0002 \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Trained}} \\
\addlinespace[1pt]
\multirow{2}{*}{\hspace*{0.75em}AR-LLM (Qwen2.5-7B)}
& 0.0018
& 0.0027
& 0.0046
& 0.0014
& 0.0018
& 0.0024 \\
& {\scriptsize (0.0017)}
& {\scriptsize (0.0025)}
& {\scriptsize (0.0041)}
& {\scriptsize (0.0013)}
& {\scriptsize (0.0017)}
& {\scriptsize (0.0022)} \\
\multirow{2}{*}{\hspace*{0.75em}MDLM (Dream-7B-Base)}
& \textbf{0.0367}
& \textbf{0.0446}
& \textbf{0.0573}
& \textbf{0.0319}
& \textbf{0.0352}
& \textbf{0.0393} \\
& {\scriptsize\textbf{(0.0366)}}
& {\scriptsize\textbf{(0.0444)}}
& {\scriptsize\textbf{(0.0569)}}
& {\scriptsize\textbf{(0.0318)}}
& {\scriptsize\textbf{(0.0351)}}
& {\scriptsize\textbf{(0.0391)}} \\
\multirow{2}{*}{\hspace*{0.75em}DiffGRM (Dream-7B-Base)}
& 0.0098
& 0.0130
& 0.0194
& 0.0074
& 0.0088
& 0.0108 \\
& {\scriptsize (0.0097)}
& {\scriptsize (0.0128)}
& {\scriptsize (0.0190)}
& {\scriptsize (0.0073)}
& {\scriptsize (0.0087)}
& {\scriptsize (0.0106)} \\
\rowcolor[HTML]{F0F8FF}
& \underline{0.0334}
& \underline{0.0409}
& \underline{0.0546}
& \underline{0.0280}
& \underline{0.0310}
& \underline{0.0354} \\
\rowcolor[HTML]{F0F8FF}
\multirow{-2}{*}{\hspace*{0.75em}HPD (Dream-7B-Base)}
& {\scriptsize\underline{(0.0333)}}
& {\scriptsize\underline{(0.0407)}}
& {\scriptsize\underline{(0.0542)}}
& {\scriptsize\underline{(0.0279)}}
& {\scriptsize\underline{(0.0309)}}
& {\scriptsize\underline{(0.0352)}} \\
\midrule
\multicolumn{7}{@{}l}{\textbf{Baby Products}} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Base model}} \\
\addlinespace[1pt]
\hspace*{0.75em}Qwen2.5-7B
& 0.0003 & 0.0004 & 0.0007 & 0.0002 & 0.0002 & 0.0003 \\
\hspace*{0.75em}Dream-7B-Base
& 0.0002 & 0.0003 & 0.0007 & 0.0002 & 0.0002 & 0.0003 \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Trained}} \\
\addlinespace[1pt]
\multirow{2}{*}{\hspace*{0.75em}AR-LLM (Qwen2.5-7B)}
& 0.0028
& 0.0039
& 0.0060
& 0.0022
& 0.0027
& 0.0033 \\
& {\scriptsize (0.0025)}
& {\scriptsize (0.0035)}
& {\scriptsize (0.0053)}
& {\scriptsize (0.0020)}
& {\scriptsize (0.0025)}
& {\scriptsize (0.0030)} \\
\multirow{2}{*}{\hspace*{0.75em}MDLM (Dream-7B-Base)}
& \textbf{0.0207}
& \textbf{0.0264}
& \textbf{0.0374}
& \textbf{0.0171}
& \textbf{0.0194}
& \textbf{0.0230} \\
& {\scriptsize\textbf{(0.0205)}}
& {\scriptsize\textbf{(0.0261)}}
& {\scriptsize\textbf{(0.0367)}}
& {\scriptsize\textbf{(0.0169)}}
& {\scriptsize\textbf{(0.0192)}}
& {\scriptsize\textbf{(0.0227)}} \\
\multirow{2}{*}{\hspace*{0.75em}DiffGRM (Dream-7B-Base)}
& 0.0050
& 0.0077
& 0.0125
& 0.0037
& 0.0048
& 0.0063 \\
& {\scriptsize (0.0048)}
& {\scriptsize (0.0074)}
& {\scriptsize (0.0118)}
& {\scriptsize (0.0035)}
& {\scriptsize (0.0046)}
& {\scriptsize (0.0060)} \\
\rowcolor[HTML]{F0F8FF}
& \underline{0.0178}
& \underline{0.0234}
& \underline{0.0331}
& \underline{0.0143}
& \underline{0.0167}
& \underline{0.0198} \\
\rowcolor[HTML]{F0F8FF}
\multirow{-2}{*}{\hspace*{0.75em}HPD (Dream-7B-Base)}
& {\scriptsize\underline{(0.0176)}}
& {\scriptsize\underline{(0.0231)}}
& {\scriptsize\underline{(0.0324)}}
& {\scriptsize\underline{(0.0141)}}
& {\scriptsize\underline{(0.0165)}}
& {\scriptsize\underline{(0.0195)}} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/qwen_llada.tex <==
\begin{table}[t]
\centering
\caption{Recommendation results for the Qwen3/LLaDA model pair on the Industrial and Scientific, Office Products, and Baby Products domains. \emph{Before} denotes inference immediately after adding the new SID tokens to the model's embedding and output spaces, prior to recommendation training. For each trained model, the smaller parenthesized value is the difference from its corresponding \emph{Before} score; positive values denote improvement. The best and second-best distinct scores within each domain and training scope are shown in \textbf{bold} and with \underline{underlining}, respectively; ties receive the same emphasis. All trained results use the checkpoint saved at update 1,000.}
\label{tab:qwen_llada_results}
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}clcccccc@{}}
\toprule
\textbf{Training scope} & \textbf{Method}
& \textbf{HR@3} & \textbf{HR@5} & \textbf{HR@10}
& \textbf{NDCG@3} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Industrial and Scientific}} \\
\addlinespace[2pt]
\multirow{2}{*}{Before}
& AR-LLM (Qwen3-8B)
& 0.0000 & 0.0004 & 0.0012 & 0.0000 & 0.0002 & 0.0004 \\
& dLLM (LLaDA-8B-Base)
& 0.0005 & 0.0009 & 0.0021 & 0.0005 & 0.0006 & 0.0010 \\
\addlinespace[2pt]
\multirow{6}{*}{SID parameters only}
& \multirow{2}{*}{AR-LLM (Qwen3-8B)}
& 0.0069
& 0.0117
& 0.0232
& 0.0053
& 0.0072
& 0.0109 \\
&
& {\scriptsize (0.0069)}
& {\scriptsize (0.0113)}
& {\scriptsize (0.0220)}
& {\scriptsize (0.0053)}
& {\scriptsize (0.0070)}
& {\scriptsize (0.0105)} \\
& \multirow{2}{*}{HPD (LLaDA-8B-Base)}
& \underline{0.0255}
& \underline{0.0293}
& \underline{0.0351}
& \underline{0.0216}
& \underline{0.0231}
& \underline{0.0250} \\
&
& {\scriptsize\underline{(0.0250)}}
& {\scriptsize\underline{(0.0284)}}
& {\scriptsize\underline{(0.0330)}}
& {\scriptsize\underline{(0.0211)}}
& {\scriptsize\underline{(0.0225)}}
& {\scriptsize\underline{(0.0240)}} \\
& \multirow{2}{*}{MDLM (LLaDA-8B-Base)}
& \textbf{0.0284}
& \textbf{0.0316}
& \textbf{0.0355}
& \textbf{0.0225}
& \textbf{0.0238}
& \textbf{0.0251} \\
&
& {\scriptsize\textbf{(0.0279)}}
& {\scriptsize\textbf{(0.0307)}}
& {\scriptsize\textbf{(0.0334)}}
& {\scriptsize\textbf{(0.0220)}}
& {\scriptsize\textbf{(0.0232)}}
& {\scriptsize\textbf{(0.0241)}} \\
\addlinespace[2pt]
\multirow{6}{*}{All model parameters}
& \multirow{2}{*}{AR-LLM (Qwen3-8B)}
& 0.0092
& 0.0129
& 0.0261
& 0.0071
& 0.0086
& 0.0128 \\
&
& {\scriptsize (0.0092)}
& {\scriptsize (0.0125)}
& {\scriptsize (0.0249)}
& {\scriptsize (0.0071)}
& {\scriptsize (0.0084)}
& {\scriptsize (0.0124)} \\
& \multirow{2}{*}{HPD (LLaDA-8B-Base)}
& \textbf{0.0266}
& \textbf{0.0309}
& \textbf{0.0374}
& \textbf{0.0239}
& \textbf{0.0256}
& \textbf{0.0277} \\
&
& {\scriptsize\textbf{(0.0261)}}
& {\scriptsize\textbf{(0.0300)}}
& {\scriptsize\textbf{(0.0353)}}
& {\scriptsize\textbf{(0.0234)}}
& {\scriptsize\textbf{(0.0250)}}
& {\scriptsize\textbf{(0.0267)}} \\
& \multirow{2}{*}{MDLM (LLaDA-8B-Base)}
& \underline{0.0161}
& \underline{0.0207}
& \underline{0.0289}
& \underline{0.0123}
& \underline{0.0142}
& \underline{0.0168} \\
&
& {\scriptsize\underline{(0.0156)}}
& {\scriptsize\underline{(0.0198)}}
& {\scriptsize\underline{(0.0268)}}
& {\scriptsize\underline{(0.0118)}}
& {\scriptsize\underline{(0.0136)}}
& {\scriptsize\underline{(0.0158)}} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Office Products}} \\
\addlinespace[2pt]
\multirow{2}{*}{Before}
& AR-LLM (Qwen3-8B)
& 0.0002 & 0.0004 & 0.0008 & 0.0002 & 0.0002 & 0.0004 \\
& dLLM (LLaDA-8B-Base)
& 0.0001 & 0.0002 & 0.0004 & 0.0001 & 0.0001 & 0.0002 \\
\addlinespace[2pt]
\multirow{6}{*}{SID parameters only}
& \multirow{2}{*}{AR-LLM (Qwen3-8B)}
& \textbf{0.0019}
& \textbf{0.0030}
& \textbf{0.0056}
& \textbf{0.0014}
& \textbf{0.0019}
& \textbf{0.0027} \\
&
& {\scriptsize\textbf{(0.0017)}}
& {\scriptsize\textbf{(0.0026)}}
& {\scriptsize\textbf{(0.0048)}}
& {\scriptsize\textbf{(0.0012)}}
& {\scriptsize\textbf{(0.0017)}}
& {\scriptsize\textbf{(0.0023)}} \\
& \multirow{2}{*}{HPD (LLaDA-8B-Base)}
& 0.0011
& 0.0017
& 0.0039
& 0.0007
& 0.0010
& 0.0017 \\
&
& {\scriptsize (0.0010)}
& {\scriptsize (0.0015)}
& {\scriptsize (0.0035)}
& {\scriptsize (0.0006)}
& {\scriptsize (0.0009)}
& {\scriptsize (0.0015)} \\
& \multirow{2}{*}{MDLM (LLaDA-8B-Base)}
& \underline{0.0014}
& \underline{0.0024}
& \underline{0.0045}
& \underline{0.0010}
& \underline{0.0014}
& \underline{0.0021} \\
&
& {\scriptsize\underline{(0.0013)}}
& {\scriptsize\underline{(0.0022)}}
& {\scriptsize\underline{(0.0041)}}
& {\scriptsize\underline{(0.0009)}}
& {\scriptsize\underline{(0.0013)}}
& {\scriptsize\underline{(0.0019)}} \\
\addlinespace[2pt]
\multirow{6}{*}{All model parameters}
& \multirow{2}{*}{AR-LLM (Qwen3-8B)}
& 0.0023
& 0.0036
& 0.0065
& 0.0016
& 0.0022
& 0.0031 \\
&
& {\scriptsize (0.0021)}
& {\scriptsize (0.0032)}
& {\scriptsize (0.0057)}
& {\scriptsize (0.0014)}
& {\scriptsize (0.0020)}
& {\scriptsize (0.0027)} \\
& \multirow{2}{*}{HPD (LLaDA-8B-Base)}
& \textbf{0.0060}
& \textbf{0.0085}
& \textbf{0.0134}
& \textbf{0.0047}
& \textbf{0.0057}
& \textbf{0.0073} \\
&
& {\scriptsize\textbf{(0.0059)}}
& {\scriptsize\textbf{(0.0083)}}
& {\scriptsize\textbf{(0.0130)}}
& {\scriptsize\textbf{(0.0046)}}
& {\scriptsize\textbf{(0.0056)}}
& {\scriptsize\textbf{(0.0071)}} \\
& \multirow{2}{*}{MDLM (LLaDA-8B-Base)}
& \underline{0.0053}
& \underline{0.0075}
& \underline{0.0124}
& \underline{0.0040}
& \underline{0.0049}
& \underline{0.0064} \\
&
& {\scriptsize\underline{(0.0052)}}
& {\scriptsize\underline{(0.0073)}}
& {\scriptsize\underline{(0.0120)}}
& {\scriptsize\underline{(0.0039)}}
& {\scriptsize\underline{(0.0048)}}
& {\scriptsize\underline{(0.0062)}} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Baby Products}} \\
\addlinespace[2pt]
\multirow{2}{*}{Before}
& AR-LLM (Qwen3-8B)
& 0.0003 & 0.0004 & 0.0007 & 0.0002 & 0.0003 & 0.0003 \\
& dLLM (LLaDA-8B-Base)
& 0.0006 & 0.0009 & 0.0013 & 0.0004 & 0.0006 & 0.0007 \\
\addlinespace[2pt]
\multirow{6}{*}{SID parameters only}
& \multirow{2}{*}{AR-LLM (Qwen3-8B)}
& \underline{0.0019}
& \underline{0.0033}
& \underline{0.0062}
& \underline{0.0013}
& \underline{0.0018}
& \underline{0.0028} \\
&
& {\scriptsize\underline{(0.0016)}}
& {\scriptsize\underline{(0.0029)}}
& {\scriptsize\underline{(0.0055)}}
& {\scriptsize\underline{(0.0011)}}
& {\scriptsize\underline{(0.0015)}}
& {\scriptsize\underline{(0.0025)}} \\
& \multirow{2}{*}{HPD (LLaDA-8B-Base)}
& \textbf{0.0031}
& \textbf{0.0044}
& \textbf{0.0072}
& \textbf{0.0023}
& \textbf{0.0028}
& \textbf{0.0037} \\
&
& {\scriptsize\textbf{(0.0025)}}
& {\scriptsize\textbf{(0.0035)}}
& {\scriptsize\textbf{(0.0059)}}
& {\scriptsize\textbf{(0.0019)}}
& {\scriptsize\textbf{(0.0022)}}
& {\scriptsize\textbf{(0.0030)}} \\
& \multirow{2}{*}{MDLM (LLaDA-8B-Base)}
& \underline{0.0019}
& 0.0026
& 0.0042
& \underline{0.0013}
& 0.0017
& 0.0021 \\
&
& {\scriptsize\underline{(0.0013)}}
& {\scriptsize (0.0017)}
& {\scriptsize (0.0029)}
& {\scriptsize\underline{(0.0009)}}
& {\scriptsize (0.0011)}
& {\scriptsize (0.0014)} \\
\addlinespace[2pt]
\multirow{6}{*}{All model parameters}
& \multirow{2}{*}{AR-LLM (Qwen3-8B)}
& 0.0021
& 0.0038
& 0.0069
& \underline{0.0014}
& 0.0022
& 0.0032 \\
&
& {\scriptsize (0.0018)}
& {\scriptsize (0.0034)}
& {\scriptsize (0.0062)}
& {\scriptsize\underline{(0.0012)}}
& {\scriptsize (0.0019)}
& {\scriptsize (0.0029)} \\
& \multirow{2}{*}{HPD (LLaDA-8B-Base)}
& \textbf{0.0095}
& \textbf{0.0133}
& \textbf{0.0207}
& \textbf{0.0074}
& \textbf{0.0090}
& \textbf{0.0114} \\
&
& {\scriptsize\textbf{(0.0089)}}
& {\scriptsize\textbf{(0.0124)}}
& {\scriptsize\textbf{(0.0194)}}
& {\scriptsize\textbf{(0.0070)}}
& {\scriptsize\textbf{(0.0084)}}
& {\scriptsize\textbf{(0.0107)}} \\
& \multirow{2}{*}{MDLM (LLaDA-8B-Base)}
& \underline{0.0092}
& \underline{0.0125}
& \underline{0.0202}
& \textbf{0.0074}
& \underline{0.0087}
& \underline{0.0112} \\
&
& {\scriptsize\underline{(0.0086)}}
& {\scriptsize\underline{(0.0116)}}
& {\scriptsize\underline{(0.0189)}}
& {\scriptsize\textbf{(0.0070)}}
& {\scriptsize\underline{(0.0081)}}
& {\scriptsize\underline{(0.0105)}} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/qwen_llada_stage1.tex <==
\begin{table}[t]
\centering
\caption{Recommendation results for the Qwen3/LLaDA model pair before recommendation training and after training only the SID-token embeddings and output weights on the Industrial and Scientific, Office Products, and Baby Products domains. Parenthesized values for trained models are differences from the corresponding base-model results. The best trained score within each domain is shown in \textbf{bold}. All trained results use the checkpoint saved at update 1,000.}
\label{tab:qwen_llada_stage1_results}
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}clcccccc@{}}
\toprule
\textbf{Training scope} & \textbf{Method}
& \textbf{HR@3} & \textbf{HR@5} & \textbf{HR@10}
& \textbf{NDCG@3} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Industrial and Scientific}} \\
\addlinespace[2pt]
\multirow{2}{*}{Before}
& OpenOneRec (Qwen3-8B)
& 0.0000 & 0.0004 & 0.0012 & 0.0000 & 0.0002 & 0.0004 \\
& Ours (LLaDA-8B-Base)
& 0.0005 & 0.0009 & 0.0021 & 0.0005 & 0.0006 & 0.0010 \\
\addlinespace[2pt]
\multirow{6}{*}{SID parameters only}
& \multirow{2}{*}{OpenOneRec (Qwen3-8B)}
& 0.0069
& 0.0117
& 0.0232
& 0.0053
& 0.0072
& 0.0109 \\
&
& {\scriptsize (0.0069)}
& {\scriptsize (0.0113)}
& {\scriptsize (0.0220)}
& {\scriptsize (0.0053)}
& {\scriptsize (0.0070)}
& {\scriptsize (0.0105)} \\
& \multirow{2}{*}{Ours (LLaDA-8B-Base)}
& 0.0255
& 0.0293
& 0.0351
& 0.0216
& 0.0231
& 0.0250 \\
&
& {\scriptsize (0.0250)}
& {\scriptsize (0.0284)}
& {\scriptsize (0.0330)}
& {\scriptsize (0.0211)}
& {\scriptsize (0.0225)}
& {\scriptsize (0.0240)} \\
& \multirow{2}{*}{Original Diffusion (LLaDA-8B-Base)}
& \textbf{0.0284}
& \textbf{0.0316}
& \textbf{0.0355}
& \textbf{0.0225}
& \textbf{0.0238}
& \textbf{0.0251} \\
&
& {\scriptsize\textbf{(0.0279)}}
& {\scriptsize\textbf{(0.0307)}}
& {\scriptsize\textbf{(0.0334)}}
& {\scriptsize\textbf{(0.0220)}}
& {\scriptsize\textbf{(0.0232)}}
& {\scriptsize\textbf{(0.0241)}} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Office Products}} \\
\addlinespace[2pt]
\multirow{2}{*}{Before}
& OpenOneRec (Qwen3-8B)
& 0.0002 & 0.0004 & 0.0008 & 0.0002 & 0.0002 & 0.0004 \\
& Ours (LLaDA-8B-Base)
& 0.0001 & 0.0002 & 0.0004 & 0.0001 & 0.0001 & 0.0002 \\
\addlinespace[2pt]
\multirow{6}{*}{SID parameters only}
& \multirow{2}{*}{OpenOneRec (Qwen3-8B)}
& \textbf{0.0019}
& \textbf{0.0030}
& \textbf{0.0056}
& \textbf{0.0014}
& \textbf{0.0019}
& \textbf{0.0027} \\
&
& {\scriptsize\textbf{(0.0017)}}
& {\scriptsize\textbf{(0.0026)}}
& {\scriptsize\textbf{(0.0048)}}
& {\scriptsize\textbf{(0.0012)}}
& {\scriptsize\textbf{(0.0017)}}
& {\scriptsize\textbf{(0.0023)}} \\
& \multirow{2}{*}{Ours (LLaDA-8B-Base)}
& 0.0011
& 0.0017
& 0.0039
& 0.0007
& 0.0010
& 0.0017 \\
&
& {\scriptsize (0.0010)}
& {\scriptsize (0.0015)}
& {\scriptsize (0.0035)}
& {\scriptsize (0.0006)}
& {\scriptsize (0.0009)}
& {\scriptsize (0.0015)} \\
& \multirow{2}{*}{Original Diffusion (LLaDA-8B-Base)}
& 0.0014
& 0.0024
& 0.0045
& 0.0010
& 0.0014
& 0.0021 \\
&
& {\scriptsize (0.0013)}
& {\scriptsize (0.0022)}
& {\scriptsize (0.0041)}
& {\scriptsize (0.0009)}
& {\scriptsize (0.0013)}
& {\scriptsize (0.0019)} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Baby Products}} \\
\addlinespace[2pt]
\multirow{2}{*}{Before}
& OpenOneRec (Qwen3-8B)
& 0.0003 & 0.0004 & 0.0007 & 0.0002 & 0.0003 & 0.0003 \\
& Ours (LLaDA-8B-Base)
& 0.0006 & 0.0009 & 0.0013 & 0.0004 & 0.0006 & 0.0007 \\
\addlinespace[2pt]
\multirow{6}{*}{SID parameters only}
& \multirow{2}{*}{OpenOneRec (Qwen3-8B)}
& 0.0019
& 0.0033
& 0.0062
& 0.0013
& 0.0018
& 0.0028 \\
&
& {\scriptsize (0.0016)}
& {\scriptsize (0.0029)}
& {\scriptsize (0.0055)}
& {\scriptsize (0.0011)}
& {\scriptsize (0.0015)}
& {\scriptsize (0.0025)} \\
& \multirow{2}{*}{Ours (LLaDA-8B-Base)}
& \textbf{0.0031}
& \textbf{0.0044}
& \textbf{0.0072}
& \textbf{0.0023}
& \textbf{0.0028}
& \textbf{0.0037} \\
&
& {\scriptsize\textbf{(0.0025)}}
& {\scriptsize\textbf{(0.0035)}}
& {\scriptsize\textbf{(0.0059)}}
& {\scriptsize\textbf{(0.0019)}}
& {\scriptsize\textbf{(0.0022)}}
& {\scriptsize\textbf{(0.0030)}} \\
& \multirow{2}{*}{Original Diffusion (LLaDA-8B-Base)}
& 0.0019
& 0.0026
& 0.0042
& 0.0013
& 0.0017
& 0.0021 \\
&
& {\scriptsize (0.0013)}
& {\scriptsize (0.0017)}
& {\scriptsize (0.0029)}
& {\scriptsize (0.0009)}
& {\scriptsize (0.0011)}
& {\scriptsize (0.0014)} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/qwen_llada_stage2.tex <==
\begin{table}[t]
\centering
\caption{Final recommendation results for the Qwen3/LLaDA model pair.}
\label{tab:qwen_llada_final_results}
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.15}
% Set the numeric factor to the desired width; 0.8 means 80% of \linewidth.
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
\textbf{Method}
& \textbf{HR@3} & \textbf{HR@5} & \textbf{HR@10}
& \textbf{NDCG@3} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
\midrule
\multicolumn{7}{@{}l}{\textbf{Industrial and Scientific}} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Base model}} \\
\addlinespace[1pt]
\hspace*{0.75em}Qwen3-8B
& 0.0000 & 0.0004 & 0.0012 & 0.0000 & 0.0002 & 0.0004 \\
\hspace*{0.75em}LLaDA-8B-Base
& 0.0005 & 0.0009 & 0.0021 & 0.0005 & 0.0006 & 0.0010 \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Trained}} \\
\addlinespace[1pt]
\multirow{2}{*}{\hspace*{0.75em}AR-LLM (Qwen3-8B)}
& 0.0092
& 0.0129
& 0.0261
& 0.0071
& 0.0086
& 0.0128 \\
& {\scriptsize (0.0092)}
& {\scriptsize (0.0125)}
& {\scriptsize (0.0249)}
& {\scriptsize (0.0071)}
& {\scriptsize (0.0084)}
& {\scriptsize (0.0124)} \\
\multirow{2}{*}{\hspace*{0.75em}MDLM (LLaDA-8B-Base)}
& \underline{0.0161}
& \underline{0.0207}
& \underline{0.0289}
& \underline{0.0123}
& \underline{0.0142}
& \underline{0.0168} \\
& {\scriptsize\underline{(0.0156)}}
& {\scriptsize\underline{(0.0198)}}
& {\scriptsize\underline{(0.0268)}}
& {\scriptsize\underline{(0.0118)}}
& {\scriptsize\underline{(0.0136)}}
& {\scriptsize\underline{(0.0158)}} \\
\rowcolor[HTML]{F0F8FF}
& \textbf{0.0266}
& \textbf{0.0309}
& \textbf{0.0374}
& \textbf{0.0239}
& \textbf{0.0256}
& \textbf{0.0277} \\
\rowcolor[HTML]{F0F8FF}
\multirow{-2}{*}{\hspace*{0.75em}HPD (LLaDA-8B-Base)}
& {\scriptsize\textbf{(0.0261)}}
& {\scriptsize\textbf{(0.0300)}}
& {\scriptsize\textbf{(0.0353)}}
& {\scriptsize\textbf{(0.0234)}}
& {\scriptsize\textbf{(0.0250)}}
& {\scriptsize\textbf{(0.0267)}} \\
\midrule
\multicolumn{7}{@{}l}{\textbf{Office Products}} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Base model}} \\
\addlinespace[1pt]
\hspace*{0.75em}Qwen3-8B
& 0.0002 & 0.0004 & 0.0008 & 0.0002 & 0.0002 & 0.0004 \\
\hspace*{0.75em}LLaDA-8B-Base
& 0.0001 & 0.0002 & 0.0004 & 0.0001 & 0.0001 & 0.0002 \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Trained}} \\
\addlinespace[1pt]
\multirow{2}{*}{\hspace*{0.75em}AR-LLM (Qwen3-8B)}
& 0.0023
& 0.0036
& 0.0065
& 0.0016
& 0.0022
& 0.0031 \\
& {\scriptsize (0.0021)}
& {\scriptsize (0.0032)}
& {\scriptsize (0.0057)}
& {\scriptsize (0.0014)}
& {\scriptsize (0.0020)}
& {\scriptsize (0.0027)} \\
\multirow{2}{*}{\hspace*{0.75em}MDLM (LLaDA-8B-Base)}
& \underline{0.0053}
& \underline{0.0075}
& \underline{0.0124}
& \underline{0.0040}
& \underline{0.0049}
& \underline{0.0064} \\
& {\scriptsize\underline{(0.0052)}}
& {\scriptsize\underline{(0.0073)}}
& {\scriptsize\underline{(0.0120)}}
& {\scriptsize\underline{(0.0039)}}
& {\scriptsize\underline{(0.0048)}}
& {\scriptsize\underline{(0.0062)}} \\
\rowcolor[HTML]{F0F8FF}
& \textbf{0.0060}
& \textbf{0.0085}
& \textbf{0.0134}
& \textbf{0.0047}
& \textbf{0.0057}
& \textbf{0.0073} \\
\rowcolor[HTML]{F0F8FF}
\multirow{-2}{*}{\hspace*{0.75em}HPD (LLaDA-8B-Base)}
& {\scriptsize\textbf{(0.0059)}}
& {\scriptsize\textbf{(0.0083)}}
& {\scriptsize\textbf{(0.0130)}}
& {\scriptsize\textbf{(0.0046)}}
& {\scriptsize\textbf{(0.0056)}}
& {\scriptsize\textbf{(0.0071)}} \\
\midrule
\multicolumn{7}{@{}l}{\textbf{Baby Products}} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Base model}} \\
\addlinespace[1pt]
\hspace*{0.75em}Qwen3-8B
& 0.0003 & 0.0004 & 0.0007 & 0.0002 & 0.0003 & 0.0003 \\
\hspace*{0.75em}LLaDA-8B-Base
& 0.0006 & 0.0009 & 0.0013 & 0.0004 & 0.0006 & 0.0007 \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Trained}} \\
\addlinespace[1pt]
\multirow{2}{*}{\hspace*{0.75em}AR-LLM (Qwen3-8B)}
& 0.0021
& 0.0038
& 0.0069
& \underline{0.0014}
& 0.0022
& 0.0032 \\
& {\scriptsize (0.0018)}
& {\scriptsize (0.0034)}
& {\scriptsize (0.0062)}
& {\scriptsize\underline{(0.0012)}}
& {\scriptsize (0.0019)}
& {\scriptsize (0.0029)} \\
\multirow{2}{*}{\hspace*{0.75em}MDLM (LLaDA-8B-Base)}
& \underline{0.0092}
& \underline{0.0125}
& \underline{0.0202}
& \textbf{0.0074}
& \underline{0.0087}
& \underline{0.0112} \\
& {\scriptsize\underline{(0.0086)}}
& {\scriptsize\underline{(0.0116)}}
& {\scriptsize\underline{(0.0189)}}
& {\scriptsize\textbf{(0.0070)}}
& {\scriptsize\underline{(0.0081)}}
& {\scriptsize\underline{(0.0105)}} \\
\rowcolor[HTML]{F0F8FF}
& \textbf{0.0095}
& \textbf{0.0133}
& \textbf{0.0207}
& \textbf{0.0074}
& \textbf{0.0090}
& \textbf{0.0114} \\
\rowcolor[HTML]{F0F8FF}
\multirow{-2}{*}{\hspace*{0.75em}HPD (LLaDA-8B-Base)}
& {\scriptsize\textbf{(0.0089)}}
& {\scriptsize\textbf{(0.0124)}}
& {\scriptsize\textbf{(0.0194)}}
& {\scriptsize\textbf{(0.0070)}}
& {\scriptsize\textbf{(0.0084)}}
& {\scriptsize\textbf{(0.0107)}} \\
\bottomrule
\end{tabular}%
}
\end{table}

